On the Role of Fault Localization Context for LLM-Based Program Repair

Fault Localization (FL) is a key component of Large Language Model (LLM)-based Automated Program Repair (APR), yet its impact remains underexplored. In particular, it is unclear how much localization is needed, whether additional context beyond the predicted buggy location is beneficial, and how such context should be retrieved. We conduct a large-scale empirical study on 500 SWE-bench Verified instances using GPT-5-mini, evaluating 61 configurations that vary file-level, element-level, and line-level context. Our results show that more context does not consistently improve repair performance. File-level localization is the dominant factor, yielding a 15-17x improvement over a no-file baseline. Expanding file context is often associated with improved performance, with successful repairs most commonly observed in configurations with approximately 6-10 relevant files. Element-level context expansion provides conditional gains that depend strongly on the file context quality, while line-level context expansion frequently degrades performance due to noise amplification. LLM-based retrieval generally outperforms structural heuristics while using fewer files and tokens. Overall, the most effective FL context strategy typically combines a broad semantic understanding at higher abstraction levels with precise line-level localization. These findings challenge our assumption that increasing the localization context uniformly improves APR, and provide practical guidance for designing LLM-based FL strategies.

==> pics_tabs/Qualitative_comparison_RQ1.tex <==
\begin{table}[t]
\caption{Qualitative comparison between violated and non-violated cases for RQ1.}
\label{tab:rq1-qual-diff}
\centering
\small
\begin{tabular}{lcc}
\toprule
\textbf{Factor} & \textbf{Violated Cases} & \textbf{Non-Violated Cases} \\
\midrule
Are extra files needed? & No & Yes \\
Context size vs.\ bug & Over-provisioned & Appropriately sized \\
File relevance & Many irrelevant files & Mostly relevant files \\
Bug complexity & Simple, localized & Complex, multi-file \\
Model behavior & Distracted, over-generalizes & Informed, focused \\
\bottomrule
\end{tabular}
\end{table}

==> pics_tabs/RQ2_N1.tex <==
\begin{table*}[t]
\caption{
Example of Improved Functional Understanding (RQ2-N1)
(sphinx\_\_sphinx-9602).
The bug arises because literal values inside typing.Literal annotations (e.g., Literal[True]) are incorrectly treated as cross-referenceable classes, triggering nitpick warnings. Expanded-function context enables the model to correctly distinguish literal values from identifiers during cross-reference resolution.}
\label{tab:rq2-n1-sphinx9602}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}
\toprule
\textbf{GT-Function Context (Incorrect Patch)} &
\textbf{Expanded-Function Context (Correct Patch)} \\
\midrule
\textbf{Location Modified:}

\texttt{sphinx/domains/python.py :: unparse()} \\
\texttt{sphinx/domains/python.py :: annotation parsing logic}

\textcolor{green!60!black}{Cross-reference resolution logic}
&
\textbf{Location Modified:}

\texttt{sphinx/domains/python.py :: unparse()}

\textcolor{red!70!black}{Superficial rendering change}
\\
\midrule
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
- return [nodes.Text(node.value)]

+ try:
+     text = repr(node.value)
+ except Exception:
+     text = str(node.value)
+ return [nodes.literal('', text)]
\end{lstlisting}

&
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
- return [nodes.Text(node.value)]
+ return [nodes.Text(repr(node.value))]

...
+ if text in ('True', 'False'):
+     continue
+ if identifier_re.match(text):
+     result[i] = type_to_xref(text, env)
\end{lstlisting}
\\
\midrule
\textcolor{red!70!black}{
\textbf{Formatting-Based Fix.}
Prevents cross-referencing by rendering literals
as literal nodes, altering annotation formatting.}
&
\textcolor{green!60!black}{
\textbf{Pipeline-Aware Fix.}
Distinguishes literal values from identifiers
during cross-reference resolution, preserving
formatting and preventing nitpick warnings.}
\\
\bottomrule
\end{tabular}
\end{table*}

==> pics_tabs/RQ2_V1.tex <==
\begin{table*}[t]
\caption{
Example of Function Context Interference (RQ2-V1)
(sympy\_\_sympy-11618). The bug arises because distance computation ignores
extra dimensions when comparing points of unequal size. GT-function context produces a localized semantic fix by promoting dimensions, whereas expanded function context introduces misleading abstractions that enforce an incorrect type restriction.}
\label{tab:rq2-v1-sympy11618}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}
\toprule
\textbf{GT-Function Context (Correct Patch)} &
\textbf{Expanded-Function Context (Incorrect Patch)} \\
\midrule
\textbf{Location Modified:}

\texttt{sympy/geometry/point.py :: distance()}

\textcolor{green!60!black}{Correct consumer function}
&
\textbf{Location Modified:}

\texttt{sympy/geometry/point.py :: distance()}

\textcolor{red!70!black}{Incorrect semantic constraint}
\\
\midrule
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
+ p = Point(p)

+ if len(self) != len(p):
+     # pad shorter point with zeros
+     ...
+ return sqrt(sum(
+   (a - b)**2
+   for a, b in zip(a_coords, b_coords)
+ ))
\end{lstlisting}
&
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
+ p = Point(p)

+ if len(self) != len(p):
+     raise ValueError(
+       "Points must be of the same dimension"
+     )
+ return sqrt(sum(
+   (a - b)**2
+   for a, b in zip(self.args, p.args)
+ ))
\end{lstlisting}
\\
\midrule
\textcolor{green!60!black}{
\textbf{Semantic Fix.}
Promotes lower-dimensional points through zero-padding,
ensuring all coordinates contribute to distance computation.}
&
\textcolor{red!70!black}{
\textbf{Over-Restriction.}
Introduces a strict dimension check, changing intended
behavior instead of correcting coordinate handling.}
\\
\bottomrule
\end{tabular}
\end{table*}

==> pics_tabs/RQ3.3_histogram.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/rq3_lines_histograms3.pdf}
    \caption{Distribution of line counts and line-level token budgets for resolved instances under different line-selection methods. %The top row shows the distribution of the number of lines provided and the corresponding line-level token budgets for Context Window expansion, the second row is for Code Slicing expansion, and the bottom row is for LLM-based expansion. Histograms show the number of resolved instances at each value, while the overlaid cumulative curves indicate cumulative resolution coverage. Horizontal percentile markers (P50, P75, P90) denote the amount of line context required to cover 50\%, 75\%, and 90\% of resolved instances, highlighting how quickly each method reaches high-resolution coverage. Statistical outliers are removed for readability.
    }
    \label{fig:line-histograms}
\end{figure*}

==> pics_tabs/RQ3_N1.tex <==
\begin{table*}[t]
\caption{
Example of Line-Level Expansion Enabling Correct Localization (RQ3-N1)
(django\_\_django-13794).
The bug prevents concatenation between regular strings and lazy strings
(\texttt{Promise}). Limited context adds only a right-hand handler,
whereas expanded context correctly implements both \texttt{\_\_add\_\_}
and \texttt{\_\_radd\_\_}.
}
\label{tab:rq3-n1-django13794}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}
\toprule
\textbf{GT-Line Context (Incorrect Patch)} &
\textbf{Expanded-Line Context (Correct Patch)} \\
\midrule
\textbf{Location Modified:} &
\textbf{Location Modified:} \\

\texttt{django/utils/functional.py :: Promise} &
\texttt{django/utils/functional.py :: Promise} \\

\textcolor{red!70!black}{Partial operator support} &
\textcolor{green!60!black}{Complete operator semantics} \\
\midrule
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
+ def __radd__(self, other):
+     ...
+     return other + self.__cast__()
\end{lstlisting}
&
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
+ def __add__(self, other):
+     ...
+     return self.__cast__() + other

+ def __radd__(self, other):
+     ...
+     return other + self.__cast__()
\end{lstlisting}
\\
\midrule
\textcolor{red!70!black}{
\textbf{Asymmetric Fix.}
Adds only right-hand concatenation,
leaving standard addition incomplete.
}
&
\textcolor{green!60!black}{
\textbf{Semantic Fix.}
Implements symmetric addition logic,
preserving Python operator behavior.
}
\\
\bottomrule
\end{tabular}
\end{table*}

==> pics_tabs/RQ3_V1.tex <==
\begin{table*}[t]
\caption{
Example of Line Context Interference (RQ3-V1) (psf\_\_requests-1766).
The bug arises from incorrect handling of the qop directive in HTTP Digest authentication. GT-line context enables correct parsing and selection of a valid token from a comma-separated list, whereas expanded-line context applies a superficial quoting change that ignores multiple supported options.
}
\label{tab:rq3-v1-requests1766}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}
\toprule
\textbf{GT-Line Context (Correct Patch)} &
\textbf{Expanded-Line Context (Incorrect Patch)} \\
\midrule
\parbox[t]{\linewidth}{
\textbf{Location Modified:}\\
\texttt{requests/auth.py :: build\_digest\_header()}\\
\textcolor{green!60!black}{Correct token-selection logic}
}
&
\parbox[t]{\linewidth}{
\textbf{Location Modified:}\\
\texttt{requests/auth.py :: build\_digest\_header()}\\
\textcolor{red!70!black}{Hard-coded quoting change}
}
\\
\midrule
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]
+ qop_tokens = [t.strip()
+               for t in qop.split(',')]
+ if 'auth' in qop_tokens:
+     qop = 'auth'
+ else:
+     qop = qop_tokens[0]

- qop=auth
+ qop="%s" % qop
\end{lstlisting}
&
\begin{lstlisting}[language=diff,basicstyle=\ttfamily\scriptsize]

- qop=auth
+ qop="%s" % 'auth'

\end{lstlisting}
\\
\midrule
\textcolor{green!60!black}{
\textbf{Semantic Fix.}
Parses comma-separated \texttt{qop} options and selects a valid token before quoting.
}
&
\textcolor{red!70!black}{
\textbf{Superficial Fix.}
Quotes a hard-coded value without handling multiple supported options.
}
\\
\bottomrule
\end{tabular}
\end{table*}
